ACE: A Model Poisoning Attack on Contribution Evaluation Methods in Federated Learning

In Federated Learning (FL), a set of clients collaboratively train a machine learning model (called global model) without sharing their local training data. The local training data of clients is typically non-i.i.d. and heterogeneous, resulting in varying contributions from individual clients to the final performance of the global model. In response, many contribution evaluation methods were proposed, where the server could evaluate the contribution made by each client and incentivize the high-contributing clients to sustain their long-term participation in FL. Existing studies mainly focus on developing new metrics or algorithms to better measure the contribution of each client. However, the security of contribution evaluation methods of FL operating in adversarial environments is largely unexplored. In this paper, we propose the first model poisoning attack on contribution evaluation methods in FL, termed ACE. Specifically, we show that any malicious client utilizing ACE could manipulate the parameters of its local model such that it is evaluated to have a high contribution by the server, even when its local training data is indeed of low quality. We perform both theoretical analysis and empirical evaluations of ACE. Theoretically, we show our design of ACE can effectively boost the malicious client's perceived contribution when the server employs the widely-used cosine distance metric to measure contribution. Empirically, our results show ACE effectively and efficiently deceive five state-of-the-art contribution evaluation methods. In addition, ACE preserves the accuracy of the final global models on testing inputs. We also explore six countermeasures to defend ACE. Our results show they are inadequate to thwart ACE, highlighting the urgent need for new defenses to safeguard the contribution evaluation methods in FL.

==> float_element/fig_amp_coeff_cs.tex <==
\begin{figure}[h]
\captionsetup{captionskip=0pt}

\centering
% \resizebox{\columnwidth}{!}{
% \includegraphics[width=\textwidth]{figs/Amplifying Coefficient-cs.pdf}
% }

\subfloat[]{
    \label{fig:capparatus}
    \centering
    \includegraphics[width=0.75\linewidth]{figs/Amp-coeff-cs.pdf}
}
% \hfill

\subfloat[]{
    \label{fig:capparatus}
    \centering
    \includegraphics[width=0.75\linewidth]{figs/Amp-coeff-acc.pdf}
}



\caption{Contribution score of the malicious client when the server uses RFFL for contribution evaluation under UNI, POW, and CLA data partitions with various amplifying coefficient $c$. The contribution score of the malicious client increases as the amplifying coefficient increases. AF is the abbreviation of Attack Free.}
\label{fig:Amp-coeff-cs}
\end{figure}



==> float_element/fig_art.tex <==
\begin{figure}[h]
\captionsetup{captionskip=0pt}

\centering
\resizebox{\columnwidth}{!}{
\includegraphics[width=\textwidth]{figs/ART.png}
}
\caption{Ratio of ART of all attack strategies compared to AF ART on three datasets.}
\label{fig:main-art}
\end{figure}



==> float_element/fig_attack_time.tex <==
\begin{figure*}[h]
    \captionsetup[subfloat]{farskip=0pt,captionskip=0pt}
    \centering
    \subfloat[CFFL-UNI]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.32\linewidth]{figs/when-attack/ab-whenattack-UNI-CFFL.pdf}
    }
    \hfill
    \subfloat[CFFL-POW]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.32\linewidth]{figs/when-attack/ab-whenattack-POW-CFFL.pdf}
    }
    \hfill
    \subfloat[CFFL-CLA]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.32\linewidth]{figs/when-attack/ab-whenattack-CLA-CFFL.pdf}
    }
    \\
    \subfloat[RFFL-UNI]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.32\linewidth]{figs/when-attack/ab-whenattack-UNI-RFFL.pdf}
    }
    \hfill
    \subfloat[RFFL-POW]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.32\linewidth]{figs/when-attack/ab-whenattack-POW-RFFL.pdf}
    }
    \hfill
    \subfloat[RFFL-CLA]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.32\linewidth]{figs/when-attack/ab-whenattack-CLA-RFFL.pdf}
    }
    
    \caption{Ablation analysis on the effect of communication round $t$ when the attacker executes \ours, with CFFL and RFFL used for contribution evaluation. The rank gain $\Delta$R is annotated by the numbers in the figure. If cosine distance is used to measure contribution (e.g., RFFL), initiating \ours~in later communication rounds can lead to higher CS. If validation accuracy is used to measure contribution (e.g., CFFL), attacking at early stage favours the attacker. }
    \label{fig:ab-attack-time}
\end{figure*}



==> float_element/fig_attacker_number_rankgain.tex <==
% \begin{figure*}[h]
%     \captionsetup[subfloat]{farskip=0pt,captionskip=0pt}
%     \centering
%     \subfloat[CFFL]{
%         \label{fig:capparatus}
%         \centering
%         \includegraphics[width=0.4\linewidth]{figs/attacker-number/rank-1-3-CFFL.pdf}
%     }
%     \hfill
%     \subfloat[RFFL]{
%         \label{fig:capparatus}
%         \centering
%         \includegraphics[width=0.4\linewidth]{figs/attacker-number/rank-1-3-RFFL.pdf}
%     }
    
    
%     \caption{The accumulated rank-gain of multiple attacker}
%     \label{fig:attacker-number-rank}
% \end{figure*}


\begin{figure}[!t]
    \captionsetup[subfloat]{farskip=0pt,captionskip=0pt}
    \centering
    % \subfloat[CFFL-UNI]{
    %     \label{fig:capparatus}
    %     \centering
    %     \includegraphics[width=0.47\columnwidth]{figs/attacker-number/cs-CFFL-UNI.pdf}
    % }
    % \hfill
    % \subfloat[RFFL-UNI]{
    %     \label{fig:capparatus}
    %     \centering
    %     \includegraphics[width=0.47\columnwidth]{figs/attacker-number/cs-RFFL-UNI.pdf}
    % }

    % \subfloat[CFFL-POW]{
    %     \label{fig:capparatus}
    %     \centering
    %     \includegraphics[width=0.47\columnwidth]{figs/attacker-number/cs-CFFL-POW.pdf}
    % }
    % \hfill
    % \subfloat[RFFL-POW]{
    %     \label{fig:capparatus}
    %     \centering
    %     \includegraphics[width=0.47\columnwidth]{figs/attacker-number/cs-RFFL-POW.pdf}
    % }
    
    \subfloat[CFFL]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.47\columnwidth]{figs/attacker-number/cs-CFFL-CLA.pdf}
    }
    \hfill
    \subfloat[RFFL]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.47\columnwidth]{figs/attacker-number/cs-RFFL-CLA.pdf}
    }

    
    \caption{This figure presents the accumulated contribution score (summation of CS of all malicious clients) under CLA data partition when the fraction of malicious clients varies from $10\%$ to $30\%$. The results indicate that \ours~is effective under different fractions of malicious clients. AF is the abbreviation of Attack Free. }
    \label{fig:attacker-number-rank}
\end{figure}



==> float_element/fig_main_accvscs.tex <==
\begin{figure*}[h]
    % \captionsetup[subfloat]{farskip=0pt,captionskip=0pt}
    \centering
    \subfloat{
    \centering
    \includegraphics[width=0.9\linewidth]{figs/main-accvscs/acc-vs-cs-legend.pdf}
    }
    \setcounter{subfigure}{0}
    \subfloat[MNIST]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=\linewidth]{figs/main-accvscs/acc-vs-cs-MNIST.pdf}
    }
    
    \subfloat[CIFAR-10]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=\linewidth]{figs/main-accvscs/acc-vs-cs-CIFAR.pdf}
    }

    \subfloat[Tiny-ImageNet]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=\linewidth]{figs/main-accvscs/acc-vs-cs-TIN.pdf}
    }    
    \caption{This figure presents the accuracy on testing inputs versus contribution score evaluated using MNIST, CIFAR-10, Tiny-ImageNet with different data partitions when the server employs different contribution evaluation methods. We observe that \ours~consistently outperforms all baselines in both dimensions when the data distribution among the clients is non-i.i.d. \JY{Could we split each figure into three? One for UNI, one for POW, and one for CLA. We could just keep one setting in main text and put the remaining two settings to Appendix? Current figures are too complex.}}
    \label{fig:acc-vs-cs}
\end{figure*}



==> float_element/fig_main_accvscs_CLA.tex <==
\begin{figure*}[h]
    % \captionsetup[subfloat]{farskip=0pt,captionskip=0pt}
    \centering
    \subfloat{
    
    \centering
    \includegraphics[width=0.5\linewidth]{figs/main-accvscs-individual/acc-vs-cs-legend-individual.pdf}
    }
    \setcounter{subfigure}{0}
    \subfloat[MNIST]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=\linewidth]{figs/main-accvscs-individual/acc-vs-cs-MNIST-CLA.pdf}
    }
    
    \subfloat[CIFAR-10]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=\linewidth]{figs/main-accvscs-individual/acc-vs-cs-CIFAR-CLA.pdf}
    }

    \subfloat[Tiny-ImageNet]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=\linewidth]{figs/main-accvscs-individual/acc-vs-cs-TIN-CLA.pdf}
    }    
    \caption{This figure presents the accuracy on testing inputs (vertical axis) versus contribution score (horizontal axis) evaluated using MNIST (first row), CIFAR-10 (second row), Tiny-ImageNet (third row) with CLA partition when the server employs different contribution evaluation methods. We observe that \ours~consistently outperforms all baselines in both dimensions when the data distribution among the clients is non-i.i.d. \JY{The figure could be polished. The number and value of y-labels are inconsistent, e.g., 4, 5, 6 y-labels. For the same row, could we make the y-label consistent (in terms of number and values)? For each column, could we make x-label consistent?} %\JY{Could we split each figure into three? One for UNI, one for POW, and one for CLA. We could just keep one setting in main text and put the remaining two settings to Appendix? Current figures are too complex.}
    }
    \label{fig:acc-vs-cs-cla}
\end{figure*}



==> float_element/fig_main_accvscs_UNI-POW.tex <==
\begin{figure*}[!htbp]
    % \captionsetup[subfloat]{farskip=0pt,captionskip=0pt}
    \centering
    \subfloat{
    \centering
    \includegraphics[width=0.5\linewidth]{figs/main-accvscs-individual/acc-vs-cs-legend-individual.pdf}
    }
    \setcounter{subfigure}{0}
    \subfloat[MNIST, UNI]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=\linewidth]{figs/main-accvscs-individual/acc-vs-cs-MNIST-UNI.pdf}
    }
    
    \subfloat[CIFAR-10, UNI]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=\linewidth]{figs/main-accvscs-individual/acc-vs-cs-CIFAR-UNI.pdf}
    }
    
    \subfloat[Tiny-ImageNet, UNI]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=\linewidth]{figs/main-accvscs-individual/acc-vs-cs-TIN-UNI.pdf}
    }
    
    \subfloat[MNIST, POW]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=\linewidth]{figs/main-accvscs-individual/acc-vs-cs-MNIST-Pow.pdf}
    }
    
    \subfloat[CIFAR-10, POW]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=\linewidth]{figs/main-accvscs-individual/acc-vs-cs-CIFAR-Pow.pdf}
    }

    \subfloat[Tiny-ImageNet, POW]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=\linewidth]{figs/main-accvscs-individual/acc-vs-cs-TIN-Pow.pdf}
    } 
    \caption{This figure presents the accuracy on testing inputs versus contribution score evaluated using MNIST, CIFAR-10, Tiny-ImageNet with UNI and POW partition when the server employs different contribution evaluation methods. We observe that \ours~consistently outperforms all baselines in both dimensions when the data distribution among the clients is non-i.i.d. }
    \label{fig:acc-vs-cs-uni-pow}
\end{figure*}



==> float_element/fig_node_number.tex <==
\begin{figure*}[htbp]
    % \captionsetup[subfloat]{farskip=0pt,captionskip=0pt}
    \centering
    \subfloat[CFFL-UNI]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.32\linewidth]{figs/node-number/ab-node-number-UNI-CFFL.pdf}
    }
    \hfill
    \subfloat[CFFL-POW]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.32\linewidth]{figs/node-number/ab-node-number-POW-CFFL.pdf}
    }
    \hfill
    \subfloat[CFFL-CLA]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.32\linewidth]{figs/node-number/ab-node-number-CLA-CFFL.pdf}
    }
    \\
    \subfloat[RFFL-UNI]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.32\linewidth]{figs/node-number/ab-node-number-UNI-RFFL.pdf}
    }
    \hfill
    \subfloat[RFFL-POW]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.32\linewidth]{figs/node-number/ab-node-number-POW-RFFL.pdf}
    }
    \hfill
    \subfloat[RFFL-CLA]{
        \label{fig:capparatus}
        \centering
        \includegraphics[width=0.32\linewidth]{figs/node-number/ab-node-number-CLA-RFFL.pdf}
    }
    
    \caption{This figure evaluates the effect of the number of clients in FL. The rank gain $\Delta R$ is annotated by the numbers in the figure. The accuracy of the global model on testing inputs does not degrade significantly under \ours~with varying client number. Regardless of the number of clients, \ours~consistently makes the attacker the highest-contributing agent. \JY{We could use a Table to show it and calculate the relative improvement in contribution score.}}
    \label{fig:ab-node-number}
\end{figure*}



==> float_element/table-hyperparameter.tex <==
\begin{table*}[hb]
\centering
\caption{This table summarizes the hyperparameters used in our experiments, which are associated with the strategies in Section \ref{sec:strategies to enhance}. In this table, $T_{LE}$ is the number of rounds for local evolution, $c$ is the amplifying coefficient, and $\Delta = \max(1,\frac{\|\mathbf{g}^t_i\|}{\|\mathbf{\hat{g}}^t\|})$.
% \JY{$T_{LE}$ is not defined. Also, what is the meaning of $c=\Delta$?}
}
\label{tab-hyperparameter}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c||cc|cc|cc||cc|cc|cc||cc|cc|cc}
\toprule 
& 
  \multicolumn{6}{c||}{MNIST} & 
  \multicolumn{6}{c||}{CIFAR-10} &
  \multicolumn{6}{c}{Tiny-ImageNet} 
   \\
&  
  \multicolumn{2}{c|}{UNI} &
  \multicolumn{2}{c|}{POW} &
  \multicolumn{2}{c||}{CLA} &
  \multicolumn{2}{c|}{UNI} &
  \multicolumn{2}{c|}{POW} &
  \multicolumn{2}{c||}{CLA} &
  \multicolumn{2}{c|}{UNI} &
  \multicolumn{2}{c|}{POW} &
  \multicolumn{2}{c}{CLA}
   \\ 
& 
  $T_{LE}$ &
  $c$ &
  
  $T_{LE}$ &
  $c$ &
  
  $T_{LE}$ &
  $c$ &
  
  $T_{LE}$ &
  $c$ &
  
  $T_{LE}$ &
  $c$ &
  
  $T_{LE}$ &
  $c$ &
  
  $T_{LE}$ &
  $c$ &
  
  $T_{LE}$ &
  $c$ &
  
  $T_{LE}$ &
  $c$ 
\\ \midrule 
FedSV  & 2 & 1 & 2 & 1 & 2 & 1 & 2 & 1 & 2 & 1 & 2 & 1 & 2 & 1 & 2 & 1 & 2 & 1 
   \\ 
LOO  & 3 & 1 & 3 & 1 & 3 & 1 & 2 & 1 & 2 & 1 & 2 & 1 & 3 & 1 & 2 & 1 & 2 & 1 
   \\ 
CFFL & 1 & 1 & 2 & 1 & 2 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 3 & 1 & 2 & 1 & 2 & 1 
   \\ 
GDR & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 
   \\ 
RFFL  & 1 & $\Delta$ & 1 & $\Delta$ & 1 & $\Delta$ & 1 & $\Delta$ & 1 & $\Delta$ & 1 & $\Delta$ & 1 & $\Delta$ & 1 & $\Delta$ & 1 & $\Delta$ 
   \\ \bottomrule
\end{tabular}%
}
\end{table*}



==> float_element/table-mainexp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


	

\newcolumntype{g}{>{\columncolor{gray!15}}c}

\begin{table*}[h]
\centering
\caption{This table summarizes the contribution score $CS$ and rank gain $\Delta R$ of the attacker when using \ours~and all baselines, evaluated under three data partitions (UNI, POW, and CLA), three datasets (MNIST, CIFAR-10, and Tiny ImageNet), and five contribution evaluation methods (FedSV, LOO, CFFL, GDR, and RFFL).
The contribution score and rank gain using \ours~consistently outperforms all baselines when the data distribution among the clients is non-i.i.d.}
\label{tab-effect-1}

\resizebox{\textwidth}{!}{%
% \addtolength{\tabcolsep}{-3pt}
% \fontsize{7}{8}\selectfont
\begin{tabular}{cc||gg|gg|gg||gg|gg|gg||gg|gg|gg}
\toprule 
&  &
  \multicolumn{6}{c||}{MNIST} & 
  \multicolumn{6}{c||}{CIFAR-10} &
  \multicolumn{6}{c}{Tiny-ImageNet} 
   \\ \rowcolor{white}
& & 
  \multicolumn{2}{c|}{UNI} &
  \multicolumn{2}{c|}{POW} &
  \multicolumn{2}{c||}{CLA} &
  \multicolumn{2}{c|}{UNI} &
  \multicolumn{2}{c|}{POW} &
  \multicolumn{2}{c||}{CLA} &
  \multicolumn{2}{c|}{UNI} &
  \multicolumn{2}{c|}{POW} &
  \multicolumn{2}{c}{CLA}
   \\ \rowcolor{white}
& &
  $CS$ &
  $\Delta R$ &
  
  $CS$ &
  $\Delta R$ &
  
  $CS$ &
  $\Delta R$ &
  
  $CS$ &
  $\Delta R$ &
  
  $CS$ &
  $\Delta R$ &
  
  $CS$ &
  $\Delta R$ &
  
  $CS$ &
  $\Delta R$ &
  
  $CS$ &
  $\Delta R$ &
  
  $CS$ &
  $\Delta R$ 
   \\ \midrule \rowcolor{white}
 &
  Attack Free & 0.0716	&0&	-0.0516&	0	&-0.2321&	0&	0.0918&	0	&-0.0237	&0&	-0.3916	&0&	-0.0672&	0&	0.0041&	0	&-0.4075	&0 
   \\ \rowcolor{white}
 & Delta Weight & 0.1142&	7	&0.1349&	6&	0.0959&	5&	0.1331&	9&	0.1355&	7&	0.1151&	5&	-0.0242&	1&	0.1091&	6&	0.1051&	5 
   \\ \rowcolor{white}
 & Data Augment. & 0.1690&	9	&0.0747&	2&	-0.3142	&0	&0.0835	&0&	0.0360&	1&	-0.4949&	0 & -0.7221	&0	&-0.0591&	0	&-0.6020&	0
   \\ \rowcolor{white}
 & Scaling Attack & -0.0067&	0&	-0.2602&	0&	-0.4442&	0&	-0.0438	&0	&-0.2700&	0&	-0.7688&	0&	-1.4040&	0&	-0.0735&	0&	-0.6458&	0 
   \\ \multirow{-5}{*}{FedSV}
 & \textbf{\ours} & 0.1295&	7&	0.1383&	6&	0.1281&	6	&0.1513&	9	&0.1367	&8&	0.1187	&5&	-0.0547&	1&	0.2650&	7	&0.2112&	6 
   \\ \midrule \rowcolor{white}
 &
  Attack Free & -0.0203&	0&	-0.1797&	0&	-1.4322	&0&	0.0508&	0&	-0.1361&	0&	-2.0367&	0&	-0.6024&	0&	-0.4143&	0&	-1.8598&	0 
   \\ \rowcolor{white}
 & Delta Weight & 0.0568&	5	&0.1439&	5&	-0.0998	&5&0.1192&	8	&0.1209&	7&	-0.0325&	5&	-0.5758&	1&	-0.0881&	5&	-0.1026&	5 
   \\ \rowcolor{white}
 & Data Augment. & 0.5084&9&-0.1527&1&-1.7173&0& 0.1004& 5& -0.0400& 0& -2.3461& 0 & -3.0225	&0	&-0.4234	&0	&-2.4076	&0
   \\ \rowcolor{white}
 & Scaling Attack & 0.4437 & 9 & -0.2144 & 0 & -1.9648 & 0 & -0.0472 & 0 & -0.4445 & 0 & -2.7999 & 0 & -5.9599 & 0 & -0.3885 & 0 & -2.3961 & 0 
   \\ \multirow{-5}{*}{LOO}
 & \textbf{\ours} & 0.3140 & 9 & 0.2602 & 8 & 0.1219 & 6 & 0.2311 & 9 & 0.1743 & 8 & -0.0003 & 5 & -0.3702 & 1 & 0.6139 & 7 & 0.4437 & 5 
   \\ \midrule \rowcolor{white}

 &

 Attack Free & 0.0995 & 0 & 0.0955 & 0 & 0.0789 & 0 & 0.0987 & 0 & 0.0860 & 0 & 0.0787 & 0 & 0.0997 & 0 & 0.0907 & 0 & 0.0816 & 0 
   
   \\ \rowcolor{white}
 & Delta Weight & 0.1005 & 9 & 0.0787 & 0 & 0.0990 & 5 & 0.1058 & 9 & 0.0715 & 0 & 0.0893 & 3 & 0.0997 & 0 & 0.0060 & 0 & 0.0805 & 0
   \\ \rowcolor{white}
 & Data Augment. & 0.0988 & 0 & 0.0941 & 0 & 0.0755 & 0 & 0.1005 & 8 & 0.0867 & 0 & 0.0813 & 1 & 0.1011 & 9 & 0.0866 & 0 & 0.0794 & 0 
   \\ \rowcolor{white}
 & Scaling Attack & 0.0961 & 0 & 0.0931 & 0 & 0.0769 & 0 & 0.0867 & 0 & 0.0795 & 0 & 0.0759 & 0 & 0.0998 & 0 & 0.0058 & 0 & 0.0791 & 0 
   \\ \multirow{-5}{*}{CFFL}
 & \textbf{\ours} & 0.1005 & 9 & 0.1008 & 7 & 0.1112 & 7 & 0.1067 & 9 & 0.1069 & 9 & 0.1152 & 8 & 0.1007 & 9 & 0.1012 & 4 & 0.1083 & 8 
   \\ \midrule \rowcolor{white}

 &
  Attack Free & 0.0935 & 0 & 0.0571 & 0 & 0.0846 & 0 & 0.0946 & 0 & 0.0489 & 0 & 0.0924 & 0 & 0.0979 & 0 & 0.0487 & 0 & 0.0824 & 0 
   
   \\ \rowcolor{white}
 & Delta Weight & 0.1651 & 9 & 0.1716 & 9 & 0.1824 & 9 & 0.2059 & 9 & 0.2111 & 9 & 0.2026 & 9 & 0.1871 & 9 & 0.1910 & 9 & 0.1940 & 9 
   \\ \rowcolor{white}
 & Data Augment. & 0.0845 & 0 & 0.0545 & 0 & 0.0718 & 0 & 0.1098 & 9 & 0.0556 & 0 & 0.0927 & 0 & 0.0997 & 4 & 0.0499 & 0 & 0.0786 & 0 
   \\ \rowcolor{white}
 & Scaling Attack & 0.0935 & 0 & 0.0571 & 0 & 0.0846 & 0 & 0.0947 & 0 & 0.0489 & 0 & 0.0924 & 0 & 0.0979 & 0 & 0.0486 & 0 & 0.0824 & 0 
   \\ \multirow{-5}{*}{GDR}
 & \textbf{\ours} & 0.1649 & 9 & 0.1717 & 9 & 0.1821 & 9 & 0.2067 & 9 & 0.2122 & 9 & 0.2043 & 9 & 0.1972 & 9 & 0.2013 & 9 & 0.2042 & 9 
   \\ \midrule \rowcolor{white}
 &
  Attack Free & 0.0840 & 0 & 0.0411 & 0 & 0.0722 & 0 & 0.0957 & 0 & 0.0451 & 0 & 0.0928 & 0 & 0.0981 & 0 & 0.0285 & 0 & 0.0783 & 0 
   
   \\ \rowcolor{white}
 & Delta Weight & 0.2083 & 9 & 0.2147 & 9 & 0.1730 & 9 & 0.1865 & 9 & 0.1916 & 9 & 0.1838 & 9 & 0.1818 & 9 & 0.2062 & 9 & 0.1930 & 9 
   \\ \rowcolor{white}
 & Data Augment. &0.0925 & 0 & 0.0557 & 0 & 0.0722 & 0 & 0.1098 & 9 & 0.0553 & 0 & 0.0925 & 0 & 0.2064 & 9 & 0.0345 & 0 & 0.1097 & 8
   \\ \rowcolor{white}
 & Scaling Attack & 0.0970 & 2 & 0.0569 & 0 & 0.0813 & 0 & 0.0957 & 0 & 0.0484 & 0 & 0.0929 & 0 & 0.2763 & 9 & 0.0365 & 0 & 0.1513 & 9 
   \\
\multirow{-5}{*}{RFFL} & \textbf{\ours} & 0.2407 & 9 & 0.2344 & 9 & 0.1818 & 9 & 0.2071 & 9 & 0.2109 & 9 & 0.2050 & 9 & 0.2335 & 9 & 0.2264 & 9 & 0.2471 & 9 
   \\ \bottomrule
\end{tabular}%
}


\end{table*}

==> float_element/table-warmup.tex <==
\begin{table}[!h]
\centering
\caption{Ablation analysis on the preliminary iteration. Applying delta weight attack to craft the local model update or learning it from training dataset gives comparable performance in terms of accuracy, contribution score, and rank gain.}
\label{tab:ab-warmup}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cc||cc | cc}
\toprule 
& & \multicolumn{2}{c|}{CFFL} & \multicolumn{2}{c}{RFFL} \\ 
& & Delta weight attack &	Train & Delta weight attack &	Train \\ \midrule 
\multirow{3}{*}{UNI} & ACC & 70.44\%	&70.80\%&	7087\%&	70.81\%  \\
& CS & 0.1051	&0.1061	&0.2071&	0.2070 \\
& $\Delta R$ & 9&	9&	9&	9 \\ \midrule
\multirow{3}{*}{POW} & ACC & 62.03\%	&62.13\%&	70.73\%&	70.79\% \\
& CS & 0.1055	&0.1065&	0.2109&	0.2079 \\
& $\Delta R$ &  8&	9&	9	&9 \\ \midrule
\multirow{3}{*}{CLA} & ACC &  52.45\%&	52.33\%&	60.10\%&	59.09\% \\
& CS & 0.1148&	0.1141&	0.2050	&0.2036 \\
& $\Delta R$ &  8	&8&	9	&9   \\ \bottomrule
\end{tabular}%
}
\end{table}

==> float_element/table_detection_more_distributions.tex <==
\begin{table}[ht]
\color{blue}

\centering
\caption{\textcolor{blue}{This table summarizes the precision, recall, and F1-score when Multi-Krum, Trimmed-Mean, FABA, Sniper, Foolsgold, or Random Guess is employed to mitigate \ours~under non-i.i.d. data distributions (i.e., POW and CLA). We observe that none of these countermeasures are effective and adequate to defend \ours.}}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{c| c | c c c | ccc}
\toprule 
\multirow{2}{*}{\makecell{Data \\ Partition}} & \multirow{2}{*}{Countermeasure} & \multicolumn{3}{c|}{CFFL} & \multicolumn{3}{c}{RFFL} \\
& & Precision & Recall & F1-Score &  Precision & Recall & F1-Score\\ \midrule
\multirow{6}{*}{POW} & Multi-Krum &  0.017 & 0.017 & 0.017 &  0.017 & 0.017 & 0.017\\ 
& Trimmed-Mean &  0.017 & 0.017 & 0.017 &  0.017 & 0.017 & 0.017 \\
& FABA &  0.017 & 0.017 & 0.017 &  0.017 & 0.017 & 0.017 \\
& Sniper &  0.022 & 0.033 & 0.027 &  0 & 0 & N/A \\
& Foolsgold &  0 & 0 & N/A & 0 & 0 & N/A \\
& Random Guess &  0.100 & 0.100 & 0.100  & 0.100 & 0.100 & 0.100\\ 
\midrule
\multirow{6}{*}{CLA} & Multi-Krum &  0.017 & 0.017 & 0.017 &  0.017 & 0.017 & 0.017\\ 
& Trimmed-Mean &  0.017 & 0.017 & 0.017 &  0 & 0 & N/A \\
& FABA &  0.017 & 0.017 & 0.017 &  0.017 & 0.017 & 0.017 \\
& Sniper &  0.022 & 0.033 & 0.026 &  0 & 0 & N/A \\
& Foolsgold &  0 & 0 & N/A & 0 & 0 & N/A \\
& Random Guess &  0.100 & 0.100 & 0.100  & 0.100 & 0.100 & 0.100\\ 
\bottomrule
\end{tabular}%
}
\label{tab:detect_POWCLA}
\end{table}

==> tab/main_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\caption{The table contains the result for}
\label{undefined}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|ccccccccc|ccccccccc|ccccccccc}
\toprule 
&  &
  \multicolumn{9}{c}{MNIST} &
  \multicolumn{9}{c}{CIFAR 10} &
  \multicolumn{9}{c}{Tiny ImageNet} 
   \\
& &
  \multicolumn{3}{c}{UNI} &
  \multicolumn{3}{c}{POW} &
  \multicolumn{3}{c}{CLA} &
  \multicolumn{3}{c}{UNI} &
  \multicolumn{3}{c}{POW} &
  \multicolumn{3}{c}{CLA} &
  \multicolumn{3}{c}{UNI} &
  \multicolumn{3}{c}{POW} &
  \multicolumn{3}{c}{CLA}
   \\
& &
  CS &
  $\Delta$R &
  Acc &
  CS &
  $\Delta$R &
  Acc &
  CS &
  $\Delta$R &
  Acc &
  CS &
  $\Delta$R &
  Acc &
  CS &
  $\Delta$R &
  Acc &
  CS &
  $\Delta$R &
  Acc &
  CS &
  $\Delta$R &
  Acc &
  CS &
  $\Delta$R &
  Acc &
  CS &
  $\Delta$R &
  Acc 
   \\ \midrule
\multirow{5}{*}{FedSV} &
  AF & & & & & & & & & & & & & & & & & & & & & & & & & & & 
   
   \\
 & B1 & & & & & & & & & & & & & & & & & & & & & & & & & & & 
   \\
 & B2 & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\
 & B3 & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\
 & Ours & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\ \midrule
\multirow{5}{*}{LOO} &
  AF & & & & & & & & & & & & & & & & & & & & & & & & & & & 
   
   \\
 & B1 & & & & & & & & & & & & & & & & & & & & & & & & & & & 
   \\
 & B2 & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\
 & B3 & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\
 & Ours & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\ \midrule

\multirow{5}{*}{CFFL} &
  AF & 0.0995 & - & 96.83 & 0.0955 & - & 94.71 & 0.0789 & - & 79.43 & 0.0995 & - & 96.83 & 0.0955 & - & 94.71 & 0.0789 & - & 79.43 & 0.0995 & - & 96.83 & 0.0955 & - & 94.71 & 0.0789 & - & 79.43 
   
   \\
 & B1 & 0.0995 & 9 & 96.83 & 0.0955 & 9 & 94.71 & 0.0789 & 9 & 79.43 & 0.0995 & 9 & 96.83 & 0.0955 & 9 & 94.71 & 0.0789 & 9 & 79.43 & 0.0995 & 9 & 96.83 & 0.0955 & 9 & 94.71 & 0.0789 & 9 & 79.43 
   \\
 & B2 & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\
 & B3 & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\
 & Ours & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\ \midrule

\multirow{5}{*}{CDR} &
  AF & & & & & & & & & & & & & & & & & & & & & & & & & & & 
   
   \\
 & B1 & & & & & & & & & & & & & & & & & & & & & & & & & & & 
   \\
 & B2 & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\
 & B3 & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\
 & Ours & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\ \midrule
\multirow{5}{*}{RFFL} &
  AF & & & & & & & & & & & & & & & & & & & & & & & & & & & 
   
   \\
 & B1 & & & & & & & & & & & & & & & & & & & & & & & & & & & 
   \\
 & B2 & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\
 & B3 & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\
 & Ours & & & & & & & & & & & & & & & & & & & & & & & & & & &
   \\ \bottomrule
\end{tabular}%
}
\end{table}
